Certified and fast computations with shallow covariance kernels

Many techniques for data science and uncertainty quantification demand efficient tools to handle Gaussian random fields, which are defined in terms of their mean functions and covariance operators. Recently, parameterized Gaussian random fields have gained increased attention, due to their higher degree of flexibility. However, especially if the random field is parameterized through its covariance operator, classical random field discretization techniques fail or become inefficient. In this work we introduce and analyze a new and certified algorithm for the low-rank approximation of a parameterized family of covariance operators which represents an extension of the adaptive cross approximation method for symmetric positive definite matrices. The algorithm relies on an affine linear expansion of the covariance operator with respect to the parameters, which needs to be computed in a preprocessing step using, e.g., the empirical interpolation method. We discuss and test our new approach for isotropic covariance kernels, such as Mat\'ern kernels. The numerical results demonstrate the advantages of our approach in terms of computational time and confirm that the proposed algorithm provides the basis of a fast sampling procedure for parameter dependent Gaussian random fields.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
%\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}

\newsiamremark{example}{Example}

\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamremark{assumption}{Assumption}
% Sets running headers as well as PDF title and authors
\headers{Fast computations with shallow covariance kernels}{D. Kressner, J. Latz, S. Massei, and E. Ullmann}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Certified and fast computations with shallow covariance kernels\thanks{Submitted to the editors DATE.
\funding{Jonas Latz and Elisabeth Ullmann acknowledge the support by Deutsche Forschungsgemeinschaft (DFG) and Technische Universit\"at M\"unchen (TUM) through the TUM International Graduate School of Science and Engineering (IGSSE) within the project 10.02 BAYES.  The work of Stefano Massei has been supported by the SNSF research project \emph{Fast algorithms from low-rank updates}; grant number: 200020\_178806}.}}

% Authors: full names plus addresses.
\author{Daniel Kressner\thanks{MATH-ANCHP, \'Ecole Polytechnique f\'ed\'erale de Lausanne, Station 8, 1015 Lausanne, Switzerland \tt (\{daniel.kressner, stefano.massei\}@epfl.ch).}
\and Jonas Latz\thanks{Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, United Kingdom \tt (jl2160@cam.ac.uk).}
  \and Stefano Massei\footnotemark[2]
\and Elisabeth Ullmann\thanks{Zentrum Mathematik, Technische Universit\"at M\"unchen, 85748 Garching bei M\"unchen, Germany \tt (elisabeth.ullmann@ma.tum.de)}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

